Strongly interacting fermions are non-trivial yet non-glassy

Random spin systems at low temperatures are glassy and feature computational hardness in finding low-energy states. We study the random all-to-all interacting fermionic Sachdev--Ye--Kitaev (SYK) model and prove that, in contrast, (I) the low-energy states have polynomial circuit depth, yet (II) the annealed and quenched free energies agree to inverse-polynomially low temperatures, ruling out a glassy phase transition in this sense. These results are derived by showing that fermionic and spin systems significantly differ in their commutation index, which quantifies the non-commutativity of Hamiltonian terms. Our results suggest that low-temperature strongly interacting fermions, unlike spins, belong in a classically nontrivial yet quantumly easy phase.

==> annealed_old.tex <==
\section{Annealed approximation for SYK model} \label{sec:annealed}

\AC{Actually, there is a black-box result that handles nonlifshitz functions}
Consider the model
\begin{align}
\vH = \frac{1}{\sqrt{L}} \sum_{\ell=1}^{L} g_{\ell} \vB_{\ell}
\end{align}
where $g_{\ell} \sim_{i.i.d.} \mathcal{N}(0,1)$ are standard independent Gaussians and $\vB_{\ell}$ are deterministic matrices. The \emph{Gibbs state} $\vrho_\beta$ at inverse temperature $\beta$ is defined by
\begin{equation}
\vrho_\beta = \frac{\e^{-\beta \vH}}{Z_\beta} \quad , \quad Z_\beta = \tr{\e^{-\beta \vH}}
\end{equation}
where $Z_\beta$ is called the \emph{partition function} at inverse temperature $\beta$.

\begin{thm}[Piesier] Let $\phi$ be convex function, and $X$ a normalized random Gaussian vector. Then,
\begin{align}
\BE\phi( f(X)-\BE f(X) ) \le  \BE \phi(\frac{\pi}{2} X'\cdot\partial f(X) )
\end{align}    
where $X'$ is an independent copy of $X$.
\end{thm}
Thus, we apply the above for $f(X) = Z$, $\phi = \labs{\cdot}_p$ to get
\begin{align}
    \labs{Z -\BE[Z]}_p &\lesssim \labs{ \sum_i g'_i \partial_i Z(g)  }_p\\
& \lesssim \sqrt{p} \labs{\sum_i \labs{\partial_i Z}^2}_{p/2} \\
& \lesssim \sqrt{p \Delta} \labs{Z}_p 
\end{align}
implying that for small enough $p\delta$,
\begin{align}
     \labs{Z - \BE Z}_p \le \frac{C \beta \sqrt{p\Delta}}{1-C \beta \sqrt{p\Delta}} \BE Z.
\end{align}
The above uses the following self-bounding inequality for any $0<a< 1$
\begin{align}
    \labs{x-\BE[x]}_q \le a \labs{x}_q \le a \L(\labs{\BE[x]}+\labs{x-\BE[x]}_q\R)\implies    \labs{x-\BE[x]}_q \le  \frac{a}{1-a} \labs{\BE[x]}.
\end{align}
\begin{fact}[Multivariate matrix Holder for Schatten norms] \label{fact:multivariate_holder}
For any $\infty\ge p,q,r\ge 1$ such that $1/r+1/p+1/q =1$ and any square matrices $\vA,\vB,\vC,$ we have that $\norm{\vA\vB\vC}_1 \le \norm{\vA}_{p} \norm{\vB}_{q} \norm{\vC}_{r}$. 
\end{fact}

% \section{}

% \AC{I am reconstructing a simpler version here.}
% Consider the model
% \begin{align}
% \vH = \frac{1}{\sqrt{L}} \sum_{\ell=1}^{L} g_{\ell} \vB_{\ell}
% \end{align}
% where $g_{\ell} \sim_{i.i.d.} \mathcal{N}(0,1)$ are standard independent Gaussians and $\vB_{\ell}$ are deterministic matrices. The \emph{Gibbs state} $\vrho_\beta$ at inverse temperature $\beta$ is defined by
% \begin{equation}
% \vrho_\beta = \frac{\e^{-\beta \vH}}{Z_\beta} \quad , \quad Z_\beta = \tr{\e^{-\beta \vH}}
% \end{equation}
% where $Z_\beta$ is called the \emph{partition function} at inverse temperature $\beta$.

% \begin{lem}[Variance of the partition function]\label{lem:variance}
% For any fixed operator $\vX$,
% \begin{align}
% \BE\L(\tr{\vX \e^{-\beta \vH}} - \BE\tr{\vX \e^{-\beta \vH}}\R)^2 \le 2\beta^2 \cdot \Delta \cdot ||\vX||_{\infty}^2 \BE Z_\beta^2.
% \end{align}
% \end{lem}
% \begin{proof}
% Rewrite Gaussians by 
% \begin{align}
% g_{\ell} = \frac{1}{\sqrt{m}}\sum_{i = 1}^{m} g_{\ell i}.
% \end{align}
% where we will take $m\rightarrow \infty$. To avoid the mean in the variance calculation, we introduce an independent copy $\vH'$ with fresh random Gaussians ($g'$) and subtract
% \begin{align}
% \tr\vX\e^{-\beta \vH} - \tr\vX\e^{-\beta \vH'} 
% = \sum_{j = 1}^m (\tr\vX\e^{-\beta \vH_{j}} - \tr\vX\e^{-\beta \vH_{j-1}}) 
% \end{align}
% where the second line defines intermediate Hamiltonians that bridge between $\vH$ and $\vH'$
% \begin{align}
% \vH_j := \sum^j_{i=1} \vA'_i +  \sum^m_{i=j+1} \vA_i \quad \text{where}\quad \vA_i := \frac{1}{\sqrt{m}} \sum_{\ell=1}^{L} g_{\ell i}\vB_{\ell}.
% \end{align}
% By construction, the updates compose a \textit{martingale difference sequence}, that is,
% \begin{align}
% \Expect\L[ \tr\vX\e^{-\beta \vH_{j}} -\tr\vX\e^{-\beta \vH_{j-1}} \mid \vA'_{j-1},\vA_{j-1},\dots, \vA'_1,\vA_1\R] = 0 \label{eq:R'jRj}.
% \end{align}
% This point is evident because we can swap the random variables $\vA_j$ and $\vA_j'$ without changing the distribution.  To analyze the martingale, we expand the difference:
% \begin{align}
% &\L(\tr\vX\e^{-\beta \vH_{j}} - \tr\vX\e^{-\beta \vH_{j-1}}\R) = -\beta \int_0^1 \tr\vX\e^{-\beta \vH_{j}s}( \vH_j - \vH_{j-1})\e^{-\beta \vH_{j-1}(1-s)} ds\\
% &= \beta \int_0^1 \tr\vX\e^{-\beta \vH_{j}s}( \vA'_j - \vA_{j})\e^{-\beta \vH_{j-1}(1-s)} ds
% = b_j - a_j + c_j 
% \end{align}
% where
% \begin{align}
% a_j &:= \beta \tr \vX \int_0^1  \e^{-\beta \vH_{j}s} \vA_j \e^{-\beta \vH_{j}(1-s)} ds
% = \beta \tr \vA_j \int_0^1 \e^{-\beta \vH_{j}(1-s)} \vX \e^{-\beta \vH_{j}s} ds \\
% b_j &:= \beta \tr \vX \int_0^1 \e^{-\beta \vH_{j-1}s} \vA'_j \e^{-\beta \vH_{j-1}(1-s)} ds
% = \beta \tr \vA'_j \int_0^1 \e^{-\beta \vH_{j-1}(1-s)} \vX \e^{-\beta \vH_{j-1}s} ds \\
% c_j &:= \beta \tr \vX \int_0^1 (\e^{-\beta \vH_{j}s} - \e^{-\beta \vH_{j-1}s}) \vA'_j \e^{-\beta \vH_{j-1}(1-s)} ds - \beta \tr \vX \int_0^1 \e^{-\beta \vH_{j}s} \vA_j (\e^{-\beta \vH_{j-1}(1-s)} - \e^{-\beta \vH_{j}(1-s)}) ds
% %\\ &= \beta \tr \vA'_j \int_0^1 \e^{-\beta \vH_{j-1}(1-s)} \vX (\e^{-\beta \vH_{j}s} - \e^{-\beta \vH_{j-1}s}) ds - \beta \tr \vA_j \int_0^1 (\e^{-\beta \vH_{j-1}(1-s)} - \e^{-\beta \vH_{j}(1-s)}) \vX \e^{-\beta \vH_{j}s} ds
% \end{align}
% The sequences $a_j, b_j, c_j$ \textit{each} form a martingale difference sequence
% \begin{align}
% \Expect\L[ a_j,b_j,c_j \mid \vA'_{j-1},\vA_{j-1},\dots, \vA'_1,\vA_1\R] = 0.
% \end{align}
% The cases $a_j,b_j$ are trivial, and the martingale property of $c_j$ inherits from the identity $c_j = b_j-a_j + (\tr\e^{-\beta \vH_{j}} - \tr\e^{-\beta \vH_{j-1}})$.
% In particular, $c_j$ is subleading in the $m\rightarrow \infty$ limit. Therefore,
% \begin{align}
% &\BE \L(\tr\vX\e^{-\beta \vH} - \BE \tr\vX\e^{-\beta \vH}\R)^2 \\
% &= \frac{1}{2} \BE \L(\tr\vX\e^{-\beta \vH'} - \tr\vX\e^{-\beta \vH}\R)^2\\
% &= \frac{1}{2} \sum_{j=1}^m \BE (b_j-a_j+c_j)^2 &\text{(Martingale property)}\\
% &\stackrel{m \rightarrow \infty}{=} \frac{1}{2} \BE \sum_{j=1}^m  (b_j-a_j)^2 &\text{($c$ is subleading in $\frac{1}{m}$)}\\
% &\le  \BE \sum_{j=1}^m  a_j^2+b_j^2 &\text{(By $(a+b)^2 \le 2(a^2+b^2)$)}\\
% &\le 2\beta^2 \cdot \frac{1}{m}\sum_{j=1}^m \BE \sum_{i=1}^{L} \L(\tr \vB_i \int_0^1 \e^{-\beta \vH_{j}(1-s)} \vX \e^{-\beta \vH_{j}s} ds\R)^2 &\text{(By $\BE[\vA_j\otimes \vA_j]= \frac{1}{m}\sum_{i=1}^L\BE[\vB_i\otimes \vB_i]$)}\\
% &\le 2\beta^2 \cdot \Delta \cdot \BE \L|\L|\int_0^1 \e^{-\beta \vH (1-s)} \vX \e^{-\beta \vH s} ds\R|\R|_1^2 &\text{(By definition of $\Delta$)}\\
% &\le 2\beta^2 \Delta \cdot \BE \L(\int_0^1 \L|\L|\e^{-\beta \vH (1-s)} \vX \e^{-\beta \vH s}\R|\R|_1 ds\R)^2\\
% &\le 2\beta^2 \cdot \Delta \cdot \BE \L(\int_0^1 ||\e^{-\beta \vH (1-s)}||_{1/(1-s)} ||\vX||_{\infty} ||\e^{-\beta \vH s}||_{1/s} ds\R)^2 &\text{(By Fact \ref{fact:multivariate_holder})}\\
% &\le 2\beta^2 \cdot \Delta \cdot ||\vX||_{\infty} \cdot \BE \L(\int_0^1 ||\e^{-\beta \vH}||_1^{(1-s)} ||\e^{-\beta \vH}||_1^{s} ds\R)^2\\
% &\le 2\beta^2 \cdot \Delta \cdot ||\vX||_{\infty}^2 \BE Z_\beta^2
% \end{align}
% \end{proof}
% \begin{fact}[Multivariate matrix Holder for Schatten norms] \label{fact:multivariate_holder}
% For any $\infty\ge p,q,r\ge 1$ such that $1/r+1/p+1/q =1$ and any square matrices $\vA,\vB,\vC,$ we have that $\norm{\vA\vB\vC}_1 \le \norm{\vA}_{p} \norm{\vB}_{q} \norm{\vC}_{r}$. 
% \end{fact}

% \begin{fact}[Matrix Hoeffding{~\cite[Theorem 1.2]{tropp2012user}}] \label{fact:matrix_hoeffding}
% For a finite sum over $N$-dimensional Hermitian matrices $\vA_i$ with independent standard Gaussian coefficients $g_i$,
% \begin{align}
% \Pr(\big|\big|\sum_{i} g_i\vA_{i}\big|\big|_{\text{op}} \ge t) \le 2N \e^{- t^2/2\sigma}\quad \text{where}\quad \sigma := \big|\big|\sum_i \vA_i^2\big|\big|_{\text{op}}. 
% \end{align}
% \end{fact}

% If we want even sharper concentration, we could also invoke the following.
% \begin{thm}[{\cite{hit_good_lambda}}]
% \label{thm:good-lambda-moments} For scalar martingales difference sequence $d_j$ (i.e., $\Expect_{j-1}d_j:=\Expect[d_j|d_{j-1},\cdots, d_1]= 0)$, we have that 
% \begin{align}
% \left| \max_{k\le n} \labs{\sum^k_{j=1} d_j} \right|_q &\lesssim \left(\sqrt{q}\left| \sum^n_{j=1} \BE_{j-1}d^*_jd_j \right|^{1/2}_{\frac{q}{2}} +q\left|\max_{1\le j\le n} |d|_j \right|_q\right).
% \end{align}
% \end{thm}
% %This would lead to a stronger Markov-type inequality (instead of Chebychev).

% \begin{lem} For any $p\ge 2,$ 
% \begin{align}
%      \labs{\tr{\vX \e^{-\beta \vH}} - \BE\tr{\vX \e^{-\beta \vH}}}_p \le C \beta^2 \cdot \Delta \cdot ||\vX||_{\infty} \labs{Z_\beta}_p.   
% \end{align}
% \end{lem}
% \begin{proof}
% \begin{align}
% \labs{\tr\vX\e^{-\beta \vH} - \BE \tr\vX\e^{-\beta \vH}}_p
% &= \frac{1}{2} \labs{ \tr\vX\e^{-\beta \vH'} - \tr\vX\e^{-\beta \vH}}_p\\
% &= \frac{1}{2} \labs{\sum_{j=1}^m b_j-a_j+c_j}_p \\
% &\stackrel{m \rightarrow \infty}{=} \frac{1}{2} \labs{ \sum_{j=1}^m b_j-a_j}_p &\text{($c$ is subleading in $\frac{1}{m}$)}\\
% &\le \frac{1}{2} \labs{ \sum_{j=1}^m b_j}_p +\frac{1}{2}\labs{ \sum_{j=1}^m a_j}_p.
% %&\le  \BE \sum_{j=1}^m  a_j^2+b_j^2 &\text{(By $(a+b)^2 \le 2(a^2+b^2)$)}\\
% \end{align}
% By Theorem~\ref{thm:good-lambda-moments}, 
% \begin{align}
% \labs{ \sum_{j=1}^m a_j}_p &\lesssim \left(\sqrt{p}\left| \sum^m_{j=1} \BE_{j-1}\labs{a}^2_j \right|^{1/2}_{\frac{p}{2}} +pm^{1/p}\left|a_j \right|_p\right)\\
% &\stackrel{m \rightarrow \infty}{=} \left(\sqrt{p}\left| \sum^m_{j=1} \BE_{j-1}\labs{a}^2_j \right|^{1/2}_{\frac{p}{2}}\right)\\
% &\le \sqrt{p} \sqrt{\sum^m_{j=1}\left| \BE_{j-1}\labs{a}^2_j \right|_{\frac{p}{2}}}\\
% &\le \beta\sqrt{p} \cdot \sqrt{ \frac{1}{m}\sum_{j=1}^m \labs{ \sum_{i=1}^{L} \L(\tr \vB_i \int_0^1 \e^{-\beta \vH_{j}(1-s)} \vX \e^{-\beta \vH_{j}s} ds\R)^2 }_{p/2}} &\text{(By $\BE[\vA_j\otimes \vA_j]= \frac{1}{m}\sum_{i=1}^L\BE[\vB_i\otimes \vB_i]$)}\\
% &\le \beta \cdot \sqrt{p\Delta} \cdot \labs{ \L|\L|\int_0^1 \e^{-\beta \vH (1-s)} \vX \e^{-\beta \vH s} ds\R|\R|_1^2 }^{1/2}_{p/2}&\text{(By definition of $\Delta$)}\\
% &= \beta \cdot \sqrt{p\Delta} \cdot \labs{ \L|\L|\int_0^1 \e^{-\beta \vH (1-s)} \vX \e^{-\beta \vH s} ds\R|\R|_1 }_{p}&\text{(By definition of $\Delta$)}\\
% %&\le 2\beta^2 \Delta \cdot \BE \L(\int_0^1 \L|\L|\e^{-\beta \vH (1-s)} \vX \e^{-\beta \vH s}\R|\R|_1 ds\R)^2\\
% %&\le 2\beta^2 \cdot \Delta \cdot \BE \L(\int_0^1 ||\e^{-\beta \vH (1-s)}||_{1/(1-s)} ||\vX||_{\infty} ||\e^{-\beta \vH s}||_{1/s} ds\R)^2 &\text{(By Fact \ref{fact:multivariate_holder})}\\
% %&\le 2\beta^2 \cdot \Delta \cdot ||\vX||_{\infty} \cdot \BE \L(\int_0^1 ||\e^{-\beta \vH}||_1^{(1-s)} ||\e^{-\beta \vH}||_1^{s} ds\R)^2\\
% &\le \beta \cdot \sqrt{p\Delta} \cdot ||\vX||_{\infty}  \labs{Z_\beta}_p
% \end{align}
% \end{proof}

% The same bound holds for the case of $b_j$. Thus, 
% By setting $\vX = \vI,$ there is an absolute constant $C$ such that
% \begin{align}
%     \labs{Z - \BE Z}_p \le C \beta \sqrt{p\Delta} \labs{Z}_p,
% \end{align}
% implying that 
% \begin{align}
%      \labs{Z - \BE Z}_p \le \frac{C \beta \sqrt{p\Delta}}{1-C \beta \sqrt{p\Delta}} \BE Z.
% \end{align}
% The above uses the following self-bounding inequality for any $0<a< 1$
% \begin{align}
%     \labs{x-\BE[x]}_q \le a \labs{x}_q \le a \L(\labs{\BE[x]}+\labs{x-\BE[x]}_q\R)\implies    \labs{x-\BE[x]}_q \le  \frac{a}{1-a} \labs{\BE[x]}.
% \end{align}
\AC{TODO: Use the concentration to conclude it's annealed.}

Also, near the logarithmic singularity, we have the unconditional bound 
\begin{align}
    \e^{\beta\norm{\vH}} \ge Z_{\beta} \ge 1
\end{align}
and 
\begin{align}
    N \BE\e^{\beta\norm{\vH}} \ge \BE Z_{\beta}
\end{align}
% \begin{align}
%     \BE Z_{\beta} \ge \BE\e^{-\beta\norm{\vH}} \ge \e^{-\beta\BE\norm{\vH}}.\tag{By convexity of exponential $\BE[\e^{x}]\ge \e^{\BE[x]}$}
% \end{align}
Therefore, the divergence singularity is controlled by $\norm{\vH}$ 
\begin{align}
    \ln(\frac{Z_\beta}{\BE Z_\beta}) \ge -  \norm{\vH} - \ln(\BE Z_\beta),
\end{align}
so we may invoke Matrix Hoeffding to control the deviation of $\norm{\vH}$ as well as an upperbound on $\ln(\BE Z_\beta)$.
\begin{thm}[Matrix Gaussian series{~\cite[Theorem 1.2]{tropp2012user}}]
    For a finite sum over Hermitian matrices $\vA_i$ with independent standard Gaussian coefficients $g_i$,
    \begin{align}
    \Pr(\norm{\sum_{i} g_i\vA_{i}} \ge t) \le 2N \e^{- t^2/2v}\quad \text{where}\quad v := \norm{\sum_i \vA_i^2}. 
    \end{align}
\end{thm}


% \section{Old text below}
% Consider the model
% \begin{align}
% \vH = \frac{1}{\sqrt{L}} \sum_{\ell=1}^{L} g_{\ell} \vB_{\ell}
% \end{align}
% where $g_{\ell} \sim_{i.i.d.} \mathcal{N}(0,1)$ are standard independent Gaussians and $\vB_{\ell}$ are deterministic matrices. The \emph{Gibbs state} $\vrho_\beta$ at inverse temperature $\beta$ is defined by
% \begin{equation}
% \vrho_\beta = \frac{\e^{-\beta \vH}}{Z_\beta} \quad , \quad Z_\beta = \tr{\e^{-\beta \vH}}
% \end{equation}
% where $Z_\beta$ is called the \emph{partition function} at inverse temperature $\beta$.

% In this section we show that the commutation index of the terms $\vB_{\ell}$ has an important effect on the concentration properties of the random model $\vH$. Denote the commutation index by
% \begin{equation}
% \Delta := \Delta(\{\vB_{\ell}\}_{\ell=1}^L)
% \end{equation}
% To see how this quantity is relevant, we can make an initial observation:
% \begin{align}
% \sup_{\vrho} \BE_{\vH}\labs{\tr(\vH \vrho)}^2 = \frac{1}{L} \sum_{\ell=1}^L \tr(\vB_{\ell} \vrho)^2 = \Delta
% \end{align}

% The first result compares~\cite{Swingle20_SK_SYK} 
% \begin{align}
%     &\BE\ln{Z_\beta} \tag*{(The quenched free energy)}\\
%     \text{vs.}\quad &\ln{\BE Z_\beta} \tag*{(The annealed free energy)}.
% \end{align}
% In particular, the quenched free energy is physical but hard to calculate while the latter appears much easier to calculate but nonphysical. The first result is that this variance quantity controls the difference between the two.
% \begin{thm}[Quenched and annealed free energy]\label{thm:quench_annealed}
% Except with probability at most $8\beta^2\Delta / (1 - 2\beta^2\Delta)$,
% \begin{align}
% \BE \ln{Z_\beta} \le \ln \BE Z_\beta \le \frac{1 - 10 \beta^2 \Delta}{1 - 2 \beta^2 \Delta} \cdot \BE \ln{Z_\beta} + \frac{2 \beta^2 \Delta (1 + 8 \beta \sqrt{n})}{1 - 2 \beta^2 \Delta}.
% \end{align}
% \end{thm}
% Therefore, a small variance $\Delta \ll \beta^{-2} $ means that the annealed free energy well-approximates the quenched free energy, which indicates the absence of spin glass order~\cite{Swingle20_SK_SYK}.

% The next result gives concentration of expectation value of the thermal state of $\vH$ for any bounded observable $\vX$.
% \begin{thm}[Concentration of expectation values]\label{thm:concentration_expectation}
% For any fixed operator $\vX$,
% \begin{align}
% \var{\tr{\vX \vrho_\beta}} \leq ???
% \end{align}
% \end{thm}

% Finally, we can show that the energy concentrates too.
% \begin{thm}[Concentration of energy]\label{thm:concentration_energy}
% \begin{align}
% \var{\tr{\vH \vrho_\beta}} \leq ???
% \end{align}
% \end{thm}
% \AC{Could have concentration of entropy and Free energy... basically all that you would care..}
% Instantiating Theorems \ref{thm:quench_annealed}, \ref{thm:concentration_expectation}, \ref{thm:concentration_energy} with the upper bound on the commutation index of Majoranas in Theorem \ref{thm:Majorana_commutation} yields the following results for the SYK model.

% \begin{cor} \label{thm:syk_annealed}
% \emph{(SYK model is annealed.)}
% For the SYK model,
% \begin{align}
% \BE \ln{Z_\beta} \le \ln \BE Z_\beta \le \BE \ln{Z_\beta} + \mathcal{O}(\beta^2 n^{-k}) \qquad \text{except with probability $\mathcal{O}(\beta^2 n^{-k})$}
% \end{align}
% \begin{align}
% \var{\tr{\vX \vrho_\beta}} \le ??? \qquad \forall \ \vX
% \end{align}
% \begin{align}
% \var{\tr{\vH \vrho_\beta}} \le ???
% \end{align}
% \end{cor}

% The rest of the section is concerned with establishing Theorems \ref{thm:quench_annealed}, \ref{thm:concentration_expectation}, \ref{thm:concentration_energy}. The main lemma is a calculation on the variance of $\tr{\vX \e^{-\beta \vH}}$.

% \begin{lem}[Variance of the partition function]\label{lem:variance}
% For any fixed operator $\vX$,
% \begin{align}
% \BE\L(\tr{\vX \e^{-\beta \vH}} - \BE\tr{\vX \e^{-\beta \vH}}\R)^2 \le 2\beta^2 \cdot \Delta \cdot ||\vX||_{\infty}^2 \BE Z_\beta^2.
% \end{align}
% \end{lem}
% \begin{proof}
% Rewrite Gaussians by 
% \begin{align}
% g_{\ell} = \frac{1}{\sqrt{m}}\sum_{i = 1}^{m} g_{\ell i}.
% \end{align}
% where we will take $m\rightarrow \infty$. To avoid the mean in the variance calculation, we introduce an independent copy $\vH'$ with fresh random Gaussians ($g'$) and subtract
% \begin{align}
% \tr\vX\e^{-\beta \vH} - \tr\vX\e^{-\beta \vH'} 
% = \sum_{j = 1}^m (\tr\vX\e^{-\beta \vH_{j}} - \tr\vX\e^{-\beta \vH_{j-1}}) 
% \end{align}
% where the second line defines intermediate Hamiltonians that bridge between $\vH$ and $\vH'$
% \begin{align}
% \vH_j := \sum^j_{i=1} \vA'_i +  \sum^m_{i=j+1} \vA_i \quad \text{where}\quad \vA_i := \frac{1}{\sqrt{m}} \sum_{\ell=1}^{L} g_{\ell i}\vB_{\ell}.
% \end{align}
% By construction, the updates compose a \textit{martingale difference sequence}, that is,
% \begin{align}
% \Expect\L[ \tr\vX\e^{-\beta \vH_{j}} -\tr\vX\e^{-\beta \vH_{j-1}} \mid \vA'_{j-1},\vA_{j-1},\dots, \vA'_1,\vA_1\R] = 0 \label{eq:R'jRj}.
% \end{align}
% This point is evident because we can swap the random variables $\vA_j$ and $\vA_j'$ without changing the distribution.  To analyze the martingale, we expand the difference:
% \begin{align}
% &\L(\tr\vX\e^{-\beta \vH_{j}} - \tr\vX\e^{-\beta \vH_{j-1}}\R) = -\beta \int_0^1 \tr\vX\e^{-\beta \vH_{j}s}( \vH_j - \vH_{j-1})\e^{-\beta \vH_{j-1}(1-s)} ds\\
% &= \beta \int_0^1 \tr\vX\e^{-\beta \vH_{j}s}( \vA'_j - \vA_{j})\e^{-\beta \vH_{j-1}(1-s)} ds
% = b_j - a_j + c_j 
% \end{align}
% where
% \begin{align}
% a_j &:= \beta \tr \vX \int_0^1  \e^{-\beta \vH_{j}s} \vA_j \e^{-\beta \vH_{j}(1-s)} ds
% = \beta \tr \vA_j \int_0^1 \e^{-\beta \vH_{j}(1-s)} \vX \e^{-\beta \vH_{j}s} ds \\
% b_j &:= \beta \tr \vX \int_0^1 \e^{-\beta \vH_{j-1}s} \vA'_j \e^{-\beta \vH_{j-1}(1-s)} ds
% = \beta \tr \vA'_j \int_0^1 \e^{-\beta \vH_{j-1}(1-s)} \vX \e^{-\beta \vH_{j-1}s} ds \\
% c_j &:= \beta \tr \vX \int_0^1 (\e^{-\beta \vH_{j}s} - \e^{-\beta \vH_{j-1}s}) \vA'_j \e^{-\beta \vH_{j-1}(1-s)} ds - \beta \tr \vX \int_0^1 \e^{-\beta \vH_{j}s} \vA_j (\e^{-\beta \vH_{j-1}(1-s)} - \e^{-\beta \vH_{j}(1-s)}) ds
% %\\ &= \beta \tr \vA'_j \int_0^1 \e^{-\beta \vH_{j-1}(1-s)} \vX (\e^{-\beta \vH_{j}s} - \e^{-\beta \vH_{j-1}s}) ds - \beta \tr \vA_j \int_0^1 (\e^{-\beta \vH_{j-1}(1-s)} - \e^{-\beta \vH_{j}(1-s)}) \vX \e^{-\beta \vH_{j}s} ds
% \end{align}
% The sequences $a_j, b_j, c_j$ \textit{each} form a martingale difference sequence
% \begin{align}
% \Expect\L[ a_j,b_j,c_j \mid \vA'_{j-1},\vA_{j-1},\dots, \vA'_1,\vA_1\R] = 0.
% \end{align}
% The cases $a_j,b_j$ are trivial, and the martingale property of $c_j$ inherits from the identity $c_j = b_j-a_j + (\tr\e^{-\beta \vH_{j}} - \tr\e^{-\beta \vH_{j-1}})$.
% In particular, $c_j$ is subleading in the $m\rightarrow \infty$ limit. Therefore,
% \begin{align}
% &\BE \L(\tr\vX\e^{-\beta \vH} - \BE \tr\vX\e^{-\beta \vH}\R)^2 \\
% &= \frac{1}{2} \BE \L(\tr\vX\e^{-\beta \vH'} - \tr\vX\e^{-\beta \vH}\R)^2\\
% &= \frac{1}{2} \sum_{j=1}^m \BE (b_j-a_j+c_j)^2 &\text{(Martingale property)}\\
% &\stackrel{m \rightarrow \infty}{=} \frac{1}{2} \BE \sum_{j=1}^m  (b_j-a_j)^2 &\text{($c$ is subleading in $\frac{1}{m}$)}\\
% &\le  \BE \sum_{j=1}^m  a_j^2+b_j^2 &\text{(By $(a+b)^2 \le 2(a^2+b^2)$)}\\
% &\le 2\beta^2 \cdot \BE \sum_{i=1}^{L} \L(\tr \vB_i \int_0^1 \e^{-\beta \vH_{j}(1-s)} \vX \e^{-\beta \vH_{j}s} ds\R)^2 &\text{(By $\BE[\vA_j\otimes \vA_j]= \frac{1}{m}\sum_{i=1}^L\BE[\vB_i\otimes \vB_i]$)}\\
% &\le 2\beta^2 \cdot \Delta \cdot \BE \L|\L|\int_0^1 \e^{-\beta \vH (1-s)} \vX \e^{-\beta \vH s} ds\R|\R|_1^2 &\text{(By definition of $\Delta$)}\\
% &\le 2\beta^2 \Delta \cdot \BE \L(\int_0^1 \L|\L|\e^{-\beta \vH (1-s)} \vX \e^{-\beta \vH s}\R|\R|_1 ds\R)^2\\
% &\le 2\beta^2 \cdot \Delta \cdot \BE \L(\int_0^1 ||\e^{-\beta \vH (1-s)}||_{1/(1-s)} ||\vX||_{\infty} ||\e^{-\beta \vH s}||_{1/s} ds\R)^2 &\text{(By Fact \ref{fact:multivariate_holder})}\\
% &\le 2\beta^2 \cdot \Delta \cdot ||\vX||_{\infty} \cdot \BE \L(\int_0^1 ||\e^{-\beta \vH}||_1^{(1-s)} ||\e^{-\beta \vH}||_1^{s} ds\R)^2\\
% &\le 2\beta^2 \cdot \Delta \cdot ||\vX||_{\infty}^2 \BE Z_\beta^2
% \end{align}
% \end{proof}

% Theorem \ref{thm:quench_annealed} follows from setting $\vX = 1$ in Lemma \ref{lem:variance} and passing to the logarithm via Chebyshev's inequality and a norm bound on $||\vH||$.

% \begin{proof}[Proof of~\autoref{thm:quench_annealed}]
% Setting $\vX = 1$ in Lemma \ref{lem:variance} gives
% \begin{equation} \label{eq:X=1}
% \frac{\BE \L(Z_\beta - \BE Z_\beta\R)^2}{\BE Z_\beta^2} \leq 2 \beta^2 \Delta
% \end{equation}
% and Chebyshev's inequality
% \begin{equation} \label{eq:chebyshev}
% \mathbb{P}(Z_\beta / \BE{Z_\beta} \leq 1/2) \leq \frac{8 \beta^2 \Delta}{1 - 2 \beta^2 \Delta}
% \end{equation}

% Now we have
% \begin{align}
% \ln{\BE Z_\beta} &= \BE \ln{Z_\beta} -\BE \ln(Z_\beta / \BE Z_\beta)
% \end{align}
% If $Z_\beta / \BE Z_\beta \leq 1/2$ then
% \begin{align}
% - \BE \ln(Z_\beta / \BE Z_\beta) \leq \frac{\BE \L(Z_\beta - \BE Z_\beta\R)^2}{(\BE Z_\beta)^2} \leq \frac{2\beta^2 \Delta}{1- 2\beta^2 \Delta}
% \end{align}
% using Equation \ref{eq:X=1} and that $\log{x} \geq (x-1) - (x-1)^2$ for $x \geq 0.316$. On the other hand, if $Z_\beta / \BE Z_\beta > 1/2$ then always $\ln(Z_\beta / \BE Z_\beta) \geq -\beta ||\vH|| - \ln \BE Z_\beta$. By law of total probability \AC{Is there a particular math identity for "law of total probability"?}, we can write
% \begin{align}
% \ln{\BE Z_\beta} &\le \BE \ln{Z_\beta} + \BP(Z_\beta / \BE Z_\beta \leq 1/2) \cdot \frac{2\beta^2 \Delta}{1- 2\beta^2 \Delta} \\
% &\qquad\qquad\qquad + \BP(Z_\beta / \BE Z_\beta > 1/2) \cdot (\beta \BE||\vH|| + \ln{\BE Z_\beta}) \\
% &\le \BE \ln{Z_\beta} + \frac{2\beta^2 \Delta}{1- 2\beta^2 \Delta} + \frac{8 \beta^2 \Delta}{1 - 2 \beta^2 \Delta} \cdot (\beta \BE||\vH|| + \ln{\BE Z_\beta}) &\text{(Equation \ref{eq:chebyshev})}\\
% \implies \quad \ln{\BE Z_\beta} &\le \frac{1 - 10 \beta^2 \Delta}{1 - 2 \beta^2 \Delta} \cdot \BE \ln{Z_\beta} + \frac{2\beta^2 \Delta}{1- 2\beta^2 \Delta} + \frac{8 \beta^2 \Delta}{1 - 2 \beta^2 \Delta} \cdot \beta \BE||\vH||
% \end{align}

% To bound $\BE||\vH||$, we can use the matrix Hoeffding inequality.
% \begin{align}
% \BE{||\vH||} &\leq \sqrt{2\log{2}} \sqrt{n} + \int_{\sqrt{2\log{2}}\sqrt{n}}^\infty \BP(\BE{||\vH||} \geq t) \\
% &\leq \sqrt{2\log{2}} \sqrt{n} + \int_{\sqrt{2\log{2}}\sqrt{n}}^\infty 2 \exp\big(-(t^2 / 2) + n \log{2}\big) dt &\text{(Fact \ref{fact:matrix_hoeffding})} \\
% &\leq \sqrt{2\log{2}} \sqrt{n} + \int_0^\infty 2 \exp\big(-\sqrt{\log{2}/2} \sqrt{n} s\big) ds &\text{($t = \sqrt{2\log{2}}\sqrt{n} + s$)} \\
% &\leq \sqrt{2\log{2}} \sqrt{n} + \frac{2\sqrt{2}}{\sqrt{\log{2}}\sqrt{n}} \\
% &\leq 2\sqrt{n} &\text{(as long as $n\geq5$)}
% \end{align}

% Overall, we can write
% \begin{align}
% \ln{\BE Z_\beta} \le \frac{1 - 10 \beta^2 \Delta}{1 - 2 \beta^2 \Delta} \cdot \BE \ln{Z_\beta} + \frac{2 \beta^2 \Delta (1 + 8 \beta \sqrt{n})}{1 - 2 \beta^2 \Delta}
% \end{align}
% \end{proof}

% \begin{fact}[Multivariate matrix Holder for Schatten norms] \label{fact:multivariate_holder}
% For any $\infty\ge p,q,r\ge 1$ such that $1/r+1/p+1/q =1$ and any square matrices $\vA,\vB,\vC,$ we have that $\norm{\vA\vB\vC}_1 \le \norm{\vA}_{p} \norm{\vB}_{q} \norm{\vC}_{r}$. 
% \end{fact}

% \begin{fact}[Matrix Hoeffding{~\cite[Theorem 1.2]{tropp2012user}}] \label{fact:matrix_hoeffding}
% For a finite sum over $N$-dimensional Hermitian matrices $\vA_i$ with independent standard Gaussian coefficients $g_i$,
% \begin{align}
% \Pr(\big|\big|\sum_{i} g_i\vA_{i}\big|\big|_{\text{op}} \ge t) \le 2N \e^{- t^2/2\sigma}\quad \text{where}\quad \sigma := \big|\big|\sum_i \vA_i^2\big|\big|_{\text{op}}. 
% \end{align}
% \end{fact}


% \AC{Ah yes, nice catch! The logarithm can blow up near $0$. However, we do have Chebychev's inequality
% \begin{align}
%     \Pr(\labs{x} \ge \epsilon) \le \frac{\BE[ x^2]}{\epsilon^2}.
% \end{align}
% therefore, the chance that we get too close to the logarithmic singularity is also very small
% \begin{align}
%     \Pr\L(\labs{\frac{Z_\beta}{\BE Z_\beta}-1} \ge \frac{1}{2}\R) \le \frac{8\beta^2 \Delta}{1- 2\beta^2 \Delta}.
% \end{align}
% Also, near the logarithmic singularity, we have the unconditional bound 
% \begin{align}
%     \e^{\beta\norm{\vH}} \ge Z_{\beta} \ge \e^{-\beta\norm{\vH}}
% \end{align}
% and 
% \begin{align}
%     \BE\e^{\beta\norm{\vH}} \ge \BE Z_{\beta}
% \end{align}
% % \begin{align}
% %     \BE Z_{\beta} \ge \BE\e^{-\beta\norm{\vH}} \ge \e^{-\beta\BE\norm{\vH}}.\tag{By convexity of exponential $\BE[\e^{x}]\ge \e^{\BE[x]}$}
% % \end{align}
% Therefore, the divergence singularity is controlled by $\norm{\vH}$ 
% \begin{align}
%     \ln(\frac{Z_\beta}{\BE Z_\beta}) \ge -  \norm{\vH} - \ln(\BE Z_\beta),
% \end{align}
% so we may invoke Matrix Hoeffding to control the deviation of $\norm{\vH}$ as well as an upperbound on $\ln(\BE Z_\beta)$.
% \begin{thm}[Matrix Gaussian series{~\cite[Theorem 1.2]{tropp2012user}}]
%     For a finite sum over Hermitian matrices $\vA_i$ with independent standard Gaussian coefficients $g_i$,
%     \begin{align}
%     \Pr(\norm{\sum_{i} g_i\vA_{i}} \ge t) \le 2N \e^{- t^2/2v}\quad \text{where}\quad v := \norm{\sum_i \vA_i^2}. 
%     \end{align}
% \end{thm}

% If we want even sharper concentration, we could also invoke the following.
% \begin{thm}[{\cite{hit_good_lambda}}]
% \label{thm:good-lambda-moments} For scalar martingales difference sequence $d_j$ (i.e., $\Expect_{j-1}d_j:=\Expect[d_j|d_{j-1},\cdots, d_1]= 0)$, we have that 
% \begin{align}
% \left| \max_{k\le n} \labs{\sum^k_{j=1} d_j} \right|_q &\lesssim \left(\sqrt{q}\left| \sum^n_{j=1} \BE_{j-1}d^*_jd_j \right|^{1/2}_{\frac{q}{2}} +q\left|\max_{1\le j\le n} |d|_j \right|_q\right).
% \end{align}
% \end{thm}
% This would lead to a stronger Markov-type inequality (instead of Chebychev).
% This might also use the following self-bounding inequality 
% \begin{align}
%     \labs{x-\BE[x]}_q \le a \labs{x}_q \le a \L(\labs{\BE[x]}+\labs{x-\BE[x]}_q\R)
% \end{align}
% implying that
% \begin{align}
%    \labs{x-\BE[x]}_q \le  \frac{a}{1-a} \labs{\BE[x]}.
% \end{align}
% % For the energy itself, 
% % \begin{align}
% %     \L(\tr\vH_{j}\e^{-\beta \vH_{j}} - \tr\vH_{j-1}\e^{-\beta \vH_{j-1}}\R)
% % \end{align}
% }



